TimeChat: A Time-sensitive Multimodal Large Language Model for Long Video Understanding

This work proposes TimeChat, a time-sensitive multimodal large language model specifically designed for long video understanding. Our model incorporates two key architectural contributions: (1) a timestamp-aware frame encoder that binds visual content with the timestamp of each frame, and (2) a sliding video Q-Former that produces a video token sequence of varying lengths to accommodate videos of various durations. Additionally, we construct an instruction-tuning dataset, encompassing 6 tasks and a total of 125K instances, to further enhance TimeChat's instruction-following performance. Experiment results across various video understanding tasks, such as dense captioning, temporal grounding, and highlight detection, demonstrate TimeChat's strong zero-shot temporal localization and reasoning capabilities. For example, it achieves +9.2 F1 score and +2.8 CIDEr on YouCook2, +5.8 HIT@1 on QVHighlights, and +27.5 R@1 (IoU=0.5) on Charades-STA, compared to state-of-the-art video large language models, holding the potential to serve as a versatile video assistant for long-form video comprehension tasks and satisfy realistic user requirements.

==> tables/7b_vs_13b.tex <==
\begin{table}[]
\centering
\begin{adjustbox}{max width=.9\linewidth}
\begin{tabular}{@{}llll|ll|ll@{}}
\toprule
\multirow{3}{*}{Model Size} & \multicolumn{3}{c|}{Dense Captioning} & \multicolumn{2}{c|}{Highlight Detection} & \multicolumn{2}{c}{Temporal Grounding} \\
       & \multicolumn{3}{c|}{YouCook2}                 & \multicolumn{2}{c|}{QVHighlights}               & \multicolumn{2}{c}{Charades-STA}              \\ \cmidrule(l){2-8} 
      & {\small SODA\_c}   & {\small CIDEr}   & {\small F1}          & mAP                  & HIT@1        & %R@1,IoU=0.5 
                 R@1{\tiny (IoU=0.5)}          
                 & %R@1,IoU=0.7 
                 R@1{\tiny (IoU=0.7)} 
                 \\ \midrule
7B & \textbf{1.2} & \textbf{3.4} & \textbf{12.6} & \textbf{14.5} & \textbf{23.9} & 32.2 & 13.4 \\
13B & 1.1 & 3.2 & 13.7 & 11.3 & 16.2 & 33.2 & 15.2 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Zero-shot performance of 7B and 13B models.}
\label{table:7b-vs-13b}
\end{table}

==> tables/sota_dvc.tex <==
\begin{table}[t!]
\centering
\begin{adjustbox}{max width=\linewidth}

\begin{tabular}{@{}lccccc@{}}
\toprule
Model & \begin{tabular}[c]{c}
\# Video \\ PT data\end{tabular} & \begin{tabular}[c]{c}
\# Trainable \\ params.\end{tabular} & SODA\_c   & CIDEr  & F1 Score \\ \midrule
\demph{Vid2Seq}~\cite{Yang2023Vid2SeqLP}  & \demph{18M} &  \demph{314M}  & \demph{7.9} &  \demph{47.1} &  \demph{27.3}   \\
\modelname (Ours) & 11.7M & 241M & 3.4  &  11.0  &  19.5 \\ 
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Performance of various VidLLMs (7B) after fine-tuneing on YouCook2 (w/o using the \datasetname dataset).}
\label{table:ft}
\end{table}

